Building Scalable Video Understanding Benchmarks through Sports

Existing benchmarks for evaluating long video understanding falls short on two critical aspects, either lacking in scale or quality of annotations. These limitations arise from the difficulty in collecting dense annotations for long videos, which often require manually labeling each frame. In this work, we introduce an automated Annotation and Video Stream Alignment Pipeline (abbreviated ASAP). We demonstrate the generality of ASAP by aligning unlabeled videos of four different sports with corresponding freely available dense web annotations (i.e. commentary). We then leverage ASAP scalability to create LCric, a large-scale long video understanding benchmark, with over 1000 hours of densely annotated long Cricket videos (with an average sample length of ~50 mins) collected at virtually zero annotation cost. We benchmark and analyze state-of-the-art video understanding models on LCric through a large set of compositional multi-choice and regression queries. We establish a human baseline that indicates significant room for new research to explore. Our human studies indicate that ASAP can align videos and annotations with high fidelity, precision, and speed. The dataset along with the code for ASAP and baselines can be accessed here: https://asap-benchmark.github.io/.

==> figures-tex/cricket_intro.tex <==
2\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/cricket_intro-v5.pdf}
    \caption{An overview of the sport of Cricket. The figure shows a ball being bowled by a bowler to a batsman from the opposite team. The \textcolor{red}{red boxes} represents players on the fielding team while the \textcolor{orange}{orange boxes} represents players on the batting team. }
    \label{fig:cricket}
\end{figure}


==> figures-tex/multi-query-stats.tex <==

\begin{figure} [ht]
    \centering
    \includegraphics[width=\linewidth]{figures/multi_2.png}
    \includegraphics[width=\linewidth]{figures/multi_4.png}
    \includegraphics[width=\linewidth]{figures/multi_8.png}
    \includegraphics[width=\linewidth]{figures/multi_10.png}
    \captionof{figure}{Ground truth output frequencies to queries used in multi-choice queries in the train set of \lcric.}
    \label{fig:multi_query_stats}
\end{figure}

==> sections/cricket_intro.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/cricket_intro-v4.pdf}
    \caption{An overview of the sport of Cricket. The figure shows a ball being bowled by a bowler to a batsman from the opposite team. The \textcolor{red}{red boxes} represents players on the fielding team while the \textcolor{orange}{orange boxes} represents players on the batting team. }
    \label{fig:cricket}
\end{figure*}

\section{3. The sport of Cricket}

In this section we provide a primer to Cricket which is widely played and watched sport, especially in east-asian countries. Here we describe basics of this sport\footnote{For a detailed explanation of all rules, a nice explainer video can also be viewed: \textit{\href{https://www.youtube.com/watch?v=AqtpNkMvj5Y}{Link}}}:

% Bullets by Yash [Start]

% This sections needs to be organized under tiny paragraphs or few statements and their headings. 

% Here's what I am thinking:
% 	a. Overview: two teams, 11 memebers each compete. 
% 	b. Bowling and Fieldling team: all members on ground, one bowler rest are fielders (catchers), explain what an over is
% 	c. Batting team: two members on the ground (called batters), hit deliveries/balls bowled by baller. 
% 	d. Goal (I think this needs most attention and good language): 
% 		i. bowling team wants to take wickets, batting team wants to score runs
% 		ii. after bowling team bowls 50 overs (in a one-day match), the team switch roles (bowling team bats, and batting team bowls) -- write better.
% 		iii. in the second half of the match, the goal for batting team is to out-score the previous team's runs in 50 overs (one-day).
% 		iv. in the second half of the match, the goal for bowling team is to prevent batting team from outscoring them. 

% Bullets by Yash [End]






\textbf{Overview:} \cric is a sport played by two teams of 11 players each that alternate between batting and fielding throughout the game. The batting team aims to score "runs" by hitting a ball that is bowled from the fielding team out of the playing field. Meanwhile, the fielding team aims to prevent the other batting team from scoring runs and dismiss all players in the batting team by hitting their wickets with the ball. Each exchange where the fielding team bowls a ball and the batting team hits the ball and attempts to score some number of runs is called a \textit{ball}, which we denote as an \textbf{atomic event} in our paper because we extract ball-by-ball annotations. There are 12 possible events per ball, which are 
\begin{itemize}
    \item The batting team scores $N$ runs, where $N \in \{0,...,9\}$
    \item A wicket is taken and the current batsman gets out.
    \item A wide ball is bowled, giving the batting team an extra run and another ball.
\end{itemize}

\textbf{Bowling Phase:} All 11 players on the fielding team stay on the field. One of the players is designated as the bowler, and their job is to deliver the ball to the batter on the batting team. The rest of the players on the fielding team are fielders (as can be seen in Fig \ref{fig:cricket} (b). If the ball is struck by the batsman, the fielders try to prevent the ball from reaching the boundary of the field and return the ball back to the pitch area. An over consists of six deliveries bowled by the same player, and each team delivers a set number of overs depending on the tournament type in their bowling phase. 

\textbf{Batting Phase:} Only two players on the batting team stay on the field at a time (see Fig \ref{fig:cricket} (b)). The batsman's job is to score runs and defend their wickets. A single run is scored when the batsman hits the ball and runs from one end of the pitch to another. Another way to score runs is to hit the ball to the boundary of the field, as shown in \ref{fig:cricket} (a), which is called the \textbf{'boundary'}, giving 4 or 6 runs to the batting team. In total, each batting team has 10 wickets. By the end of the game, the team with the most runs scored wins. 

% \textbf{Atomic Events for our dataset:} For the creation of our dataset, we use atomic events (the result of a ball) to build the queries for testing a model's reasoning capacity. In total there are \textit{12 atomic events} that we consider for building queries to build our dataset, namely the \textbf{runs scored (0-9), wicket (W), wide(w)}. Here `wide' refers to a foul leading to an extra run and ball being given to the batting team.

% These two players take turn at hitting the deliveries bowled by opposing team's bowlers. to be continued....  


% For getting an \LVU dataset, we focus on the sport of Cricket. Fig \ref{fig:cricket} shows some of the key components/actions of the game. In the game at a time, two teams (comprising of 11 players each) compete with each other, with both taking turns for batting while the other team bowls. A \textit{ball} being played is the most basic event in a match and result of this is termed as an \textbf{atomic event}. The result of a ball is often  `runs' (scores) being scored by the batting team and the team with the greater total tally of runs is considered to have won. Often there are a certain number of \textbf{`overs'} being played by each team depending on the tournament type, with an over being a collection of 6 balls. Fig \ref{fig:cricket} (b) shows the playing pitch with the batter and bowler. The aim for the batting team is to hit the ball and hence score runs which they can acquire by hitting the ball and then running from end of the pitch to another as can be seen in Fig \ref{fig:cricket} (c). 
% Another way to score runs is to hit the ball to get to the boundary of the ground as can be seen in Fig \ref{fig:cricket} (a), which is termed as a \textbf{`boundary'} and also amounts to addition of 4/6 runs to the batting team. The aim of the bowling team is to get the playing batsman out by taking their \textbf{`wicket'} (considered as `out' or simply `wicket'), which means getting the playing batsman out. In total there are 10 wickets for each team. While there are variations in the number of runs scored, there are also variations in bowling type, one of which is \textbf{`wide'}, which is a kind of foul leading to extra run and ball being given to the batting team. In total there are \textit{12 atomic events} that we consider for building queries to build our dataset, namely the \textbf{runs scored (0-9), wicket (W), wide(w)}.

% A team is considered to have won if the total tally of "runs" (scores) acquired by them are more than the other team. Fig \ref{fig:cricket} (a) shows the ground/boundary for the game, with the main playing pitch at the centre of this. Fig \ref{fig:cricket} (b) shows the playing pitch with the players of a team batting (here the two players holding a bat) while the other teams bowls. The aim for the batting team is to hit the ball and hence score runs which they can acquire by hitting the ball and then running from end of the pitch to another as can be seen in Fig \ref{fig:cricket} (c). At the same time, for the bowler team there are "fielders" scattered around the ground to catch the ball and return it to the pitch. The aim of the bowling team is to get the playing batsman out by "taking their wicket", which can happen in multiple ways, some of them being, a direct catch by the fielder of the ball hit by the batsman, the wickets behind player being hit, etc. In total, there are 10 players that come to bat from the batting team, with the number of balls dependant on the type of tournament being played. All these ball-by-ball events are what we term as "atomic events" and we consider 12 such events for our cases. These are the runs scored in a ball from '0' to '9' (inclusive of both) and two special events being, 'wide (w)' and 'out (W)'. Here 'out' refers to the wicket being taken and 'wide' is an invalid type of ball being played by the bowler leading to an extra run and ball being awarded to the batting team.

==> sections/method.tex <==
% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/approach-v5.pdf}
%     \caption{An overview of the LCric Annotation Pipeline. \textbf{Step 1} shows the over/ball score extraction process with the bounding boxes being extracted framewise and passing them in a combined fashion through the OCR. We also see the the removal of one of the extracted balls (\textcolor{red}{Over 50}) due to its length exceeding an average ball's length because of the presence of stale information. \textbf{Step 2} shows the scraping from \href{https://www.espncricinfo.com/}{ESPNCricInfo} and matching the over-wise annotations from previous step to get an event chain. \textbf{Step 3} shows the formation of our query set on an example event chain. The resultant answer of the 3 example queries (marked as \textcolor{red}{red}, \textcolor{green}{green} and \textcolor{blue}{blue}) can be seen in their corresponding colored boxes.}
%     \label{fig:approach}
% \end{figure*}

% \begin{figure*}[htb!]
%     \centering
%     \begin{minipage}{\linewidth}
%     \begin{subfigure}[b]{0.4\textwidth}
%         \centering
%         \includegraphics[scale=0.33]{figures/stats2.png}
%         \label{fig:stats:query}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.33\textwidth}
%     \includegraphics[scale=0.33]{figures/query_stat.png}
%     \label{fig:stats:length}
%     \end{subfigure}
%     \vskip\baselineskip
%     \begin{subfigure}[b]{\textwidth}
%         \centering
%         \includegraphics[scale=0.33]{figures/stats1.png}
%         \label{fig:stats:length2}
%     \end{subfigure}
%     \end{minipage}
    
%     \caption{Different stats featured in LCric. \textbf{Top left (a)} shows the number of clips of each over-length from 1-10 in LCric. \textbf{Top Right (b)} depicts 
%     the probability of a binary query about a 10-over clip of a match in the dataset holding true. \textbf{Bottom (c)} features the distribution between clip length and over length over 1,5, and 10-over clips.}
%     \label{fig:stats}
% \end{figure*}

\section{4. The \lcric dataset \textbf{\yk{To be removed.}}}


We present \lcric{}, a large-scale video understanding benchmark, to evaluate a model's ability to localize and aggregate context over \textit{really} long videos ($\sim$1 hour long). Annotating very long videos is prohibitively expensive and serves as a major challenge in collecting a large-scale video dataset. To mitigate this obstacle, we first observe that sports matches tend to provide a rich source of very long videos($\ge$1 hour per match) and also contain a diverse set of events, actions, and outcomes. To annotate these long sports matches, we develop a novel pipeline that extracts meta-data such as scorecard information from a video, then indexes and maps this information to online sports websites containing rich sets of annotations such as major events and commentary. 

We demonstrate the viability of our novel annotation pipeline by annotating \textbf{over 1000 hours} of cricket matches with annotations ranging from fine-grained ball-level information to queries that require context spanning dozens of balls. To comprehensively evaluate models on a wide range of tasks, we automatically generate around 230 diverse queries that evaluate short-term reasoning and localization (e.g. was a run scored, and did the batter get out, etc.) or long-form understanding (e.g. did two consecutive 4 runs and a wide ball occur between two outs within the first 10 overs?).

% Sport matches offer a goldmine for such kinds of data on account of their lengthy nature and also multitude of action being performed for even a single outcome to occur. We specifically focus on the sport of \textit{Cricket}, where events of the match are discretized into deliveries/balls, which define the granularity of our annotations. Within each ball, a batter can score some number of runs and hit out, wide, or nothing special. We consider the outcomes possible in a single ball as an \textit{atomic event} and build out final query set and video clips by concatenating various clips consisting of balls being played. This helps to have a varied set of clip durations that is manually tweable to test our the long-horizon capacity of any model. 

% Additionally, 6 legal balls form an over, which we use to form longer queries.

% \todo{still have to change here}

% LCric offers a dataset with queries requiring the use of context that can span from a range of few minutes to about an hour of continuous video to answer. Sport matches offer these values in the sense that to understand and reason over them, we require a large context and the rich set of actions performed in a match lends to the complexity of the problem. Specifically we focus on the sport of \textit{Cricket}, where the events of the match are discretized into deliveries/balls, which define the granularity of our annotations. We term the outcome of each ball being played as an \textit{atomic event} and similarly

% The videos are all official matches from the sport \textit{Cricket}, where the events of the match can discretized into deliveries/balls, which define the granularity of our annotations. Within each ball, a batter can score some number of runs and hit out, wide, or nothing special. Additionally, 6 legal balls form an over, which we use to form longer queries.



% The LCric dataset features a plethora of fully annotated cricket matches with annotations ranging from fine-grained ball-level information to queries that require context spanning multiple overs. The current set of annotations include a wide variety of queries that require short-term reasoning (e.g. was a run scored, and did the batter hit out, etc.) and long-form understanding of the match (e.g. did two consecutive 4 runs and a wide ball occur between two outs within the first 10 overs?). 


\subsection{Annotation Pipeline}
We leverage our novel annotation pipeline to efficiently annotate publicly-available full cricket match videos with \textit{little to no manual effort} and \textit{no annotation cost}. The annotations are derived from a popular Cricket website \href{https://www.espncricinfo.com/}{ESPNCricInfo}, which contains rich annotation for every ball for most cricket matches along with relevant player and team meta-data (statistics for individual players, teams etc.). We align these easily accessible annotations with publicly available cricket matches though our fully automated multi-stage annotation pipeline. Figure \ref{fig:approach} illustrates our annotation pipeline, which consists of three stages: (1) Extracting scorecards from videos and segmenting the video into clips for different balls, (2) Aligning video clips with Web data and (3) Generating structured queries to evaluate reasoning capabilities of models'. 

\textbf{Stage 1: Score Extraction and Ballwise Chunking}

% Yash Bullets [Start] 
% 1. Describe the scorecard (some parts are in), and how it is updated. 

% 2. Describe the overs patch-extraction, video sampling freq, and how we make it robust via matching histograms (to pertubations, point to figure), and how we club multiple OCR patches together for parallelization (this may not be so imp). Do we have stats on how many cropped patches did not return correct info

% 3. Describe ballwise chunking (point to appropiate places in figure)

% Yash Bullets [End]

% potential issues with extraction of ocr patch
% The task of aligning the web and visual data although seemingly obvious is non trivial due to the noisy nature of the screen scorecard. The score card dynamically floats on screen, may change its attributes (format, shape, color, etc.), get occluded by ads, or occasionally become stale (due to delayed updates). In this report we  detail these challenges, and our fixes for the same.

Each cricket match video contains a strip at the bottom of the screen with various metadata and information about which ball (or over) is currently being played. Hence, in a framewise fashion, we crop out the desired `over' box (with bounding box coordinates automatically generated) and extract the relevant metadata with the \texttt{Google Cloud OCR API}. The task of extracting metadata from the scorecard strip is non-trivial due to the noisy nature of the scorecard. We list some major challenges below.

% which can lead to wrong frames being passed through the OCR and getting wrong alignment in the data.

\noindent \textbf{Dynamic Floating Score card, occlusion by ads, changing attributes (format, shape, color, etc).} The score card used for the further case of 

To solve this problem of inconsistent pattern of overs score card, we employ a `reference frame', a cropped over box image, which we use to compare with all the other frames before we crop the over box region. The reference frame along with the bounding box for the over text are both automatically generated using our pipeline by randomly sampling various frames from the middle of a match and passing them through the OCR. The text with a gradual increase in its value through the frames (of 0.1 over in this case) is taken as the over text and its corresponding bounding box taken from OCR is used as the reference frame. The reference frame is compared with each prospective video frame before cropping, by using a simple average L1 distance between their pixels and using a set threshold to identify `good' frames. This helps in ignoring frames with `abnormal attributes' like moving over strip or when it gets occluded by ads. Also, having a distance function ensures the pixel value distribution of each score card resembles that of a reference frame and hence helps consistently good results from the OCR calls.

\noindent \textbf{OCR calls for each `good' frame can be expensive.} With each match lasting around 7-8 hrs and the score card changing(with each ball) every 40-50 seconds on average, passing all the 'good' frames through the OCR can be a really expensive operation. To improve on this, we stack all the score card boxes in a single image as can be seen in Fig \ref{fig:approach} \textit{Step 1}. Since a ball lasts upto 40-50 seconds ($\sim$1000 frames), we also skip various different instances of the same ball in this stacked representation by again using a simple L1 distance function between consecutive frames.

% \textbf{Challenges: }
% The score card dynamically floats on screen, may change its attributes (format, shape, color, etc.), get occluded by ads, or occasionally become stale (due to delayed updates). Because of all these variations, there is a high chance of wrong frames being passed through the OCR and hence getting wrong alignment in the data. 

% \textbf{Solutions: }
% To solve this, we employ a `reference frame', a cropped over box image, which we use to compare with all the other frames before we crop the over box region. The reference frame is randomly sampled from the middle of the match and a bounding box is generated  \textcolor{green}{The reference frame is randomly selected from the middle tup some frames from the middle and then we manually give a bounding box for the same. From that we get various prospective frames and we just select any one having a set distribution (pixel value wise)}

t
% The reference frame is selected by randomly sampling various frames and accordingly choosing one with certain nice properties (distribution-wise).

% The reference frame is compared with each prospective video frame before cropping, by using a simple average L1 distance between their pixels and using a set threshold to identify `good' frames. This helps in ignoring frames with `abnormal attributes' like moving over strip or when it gets occluded by ads. Also having a distance function ensures each score card image pixel distribution resembling that of a reference frame and hence helps in consistent good results from the OCR calls. To avoid running OCR calls on every `good' frame, we also stack all these up in a single image as can be seen in Fig \ref{fig:approach} \textit{Step 1}. Since a ball lasts upto 30-50 seconds ($\sim$1000 frames), we also skip various different instances of the same ball in this stacked representation by again using a simple L1 distance function between consecutive frames.

% Most cricket matches contain a spatially-fixed scorecard \todo{mark this in the fig} which contains information about which ball the match is at (Most scorecards have the ball information next to the "Overs" text \todo{VM: point to figure}. The pipeline extracts this information with Google OCR Vision \todo{VM: Insert link} to locate the bounding box position of the "Overs" text in a few random frames of the video. 

% Since the scorecard does not appear on every frame, we avoid running expensive OCR models on every frame by generating a reference image of a bounding box containing the "Overs" text and use simple pixel-similarity metrics \todo{equation} and simple empirical thresholding \todo{equation} to determine if a frame contains a scorecard. We then run the OCR model on frames containing the scorecard to get the start and end times of each ball in the match.

\noindent \textbf{Stage 2: Aligning extracted score information with web data} 

% Yash Bullets [Start] 

% 1. Describe the website, and how it can be obtained (scraped).
% 2. Describe alignment (ballwise)
% 3. Describe additional annotations beyond just events (natural language commentary etc).
% 4. We can also mention a snippet of commentary in figure to show how well it localizes/classifies action via free-form text.
% Yash Bullets [End]


\href{https://www.espncricinfo.com/}{ESPNCricInfo} is the largest storehouse for cricket data with various kinds of information associated with each ball. Ranging from dense event annotations like runs scored/any special event to dense natural language commentary helps us to tweak the granularity of our dataset accordingly. An example of the information can also be seen in Fig \ref{fig:approach} \textit{Step 2}, which we use to scrape the data and align with our already scraped visual data using the over numbers as the anchor, leading to the creation of an `event chain' for the whole match. An event chain is what we describe as ball-wise annotations (the runs/events associated with a ball) for the match (see Fig \ref{fig:approach} \textit{Step 2}).

% We scrape commentary and other match event annotations from ESPNCricInfo. The  ball-by-ball commentary contains information about the batter, bowler, number of runs scored, and whether a ball was hit out or wide. Additionally, the scraped information contains actual text commentary for a few matches, which may also be used as additional annotations. Coupled with the accurate timestamp information for every ball from stage 1, the scraped annotations result in rich ball-by-ball annotations for each match.

\noindent \textbf{Stage 3. Generating structured query set} 
% Yash Bullets [Start] 

% 0. Why we build queries? To study long video understanding blah blah.

% 1. Describe an event, and event chain (point in figure), maybe provide some stats of an event chain in a typical cricket match. 

% 2. 


% Yash Bullets [End]

With the presence of the event-chain for the full match, we target the long-horizon task by using various different splits of this to suit our task. As can be seen in Fig \ref{fig:approach} \textit{Step 3}, three different splits (colored as \textit{red}, \textit{green}, \textit{blue}) of an  example event chains are used for evaluation on our queries. Ranging from as small as 1 over ($\sim$5 mins) to as long as 10 overs ($\sim$50 mins), we combine ball-wise annotations to form different length event chains. To evaluate on these, we also create custom query sets for different lengths of event chains as can be seen in Fig \ref{fig:approach} \textit{Step 3}. Using different operators and combinators, we create these queries to be of different complexity and assessing different capabilities of a video understanding model. For a detailed explanation on query set formation, refer to Section \ref{sec:query_formation}.

% Since ball-level annotations comprise of a discrete set, we compose ball-level annotations across multiple balls to create a single annotation. For example, asking if "batter $A$ scored a run on ball $10.1$" is a simple ball-level query which can then be transformed into "did batter $A$ or $B$ score more over a series of contiguous balls" by aggregating the relevant ball-level annotations. Our pipeline provides scripts for generating annotations over any number of contiguous balls and can generate free high quality annotations for arbitrarily long videos. We discuss the evaluation protocol in greater detail in the following subsection.

\subsection{Query Formation}
\label{sec:query_formation}

Taking inspiration from previous works \cite{johnson2017clevr, hudson2019gqa}, we develop an automated system for evaluating the localization, aggregation, and reasoning skills of video models on our dataset. From our set of ball-by-ball annotations, we  formalize a video understanding task, which is defined as follows: Given a very long video clip (length ranging from 30 seconds to 50 minutes) and a structured query $Q$, a model is tasked to predict the right answer from either a set of options $A_1 \cdots A_N$ or predict a scalar value.

As can be seen in Fig \ref{fig:approach} \textit{Step 3}, once we have an event chain created for a whole match, we can sample various clips from the same of different lengths (1 over ($\sim$5 minutes) to 10 overs ($\sim$50 minutes)) to create a set of event chains. These event chains, combined with a set of logical operators (\texttt{atleast}, \texttt{atmost}, \texttt{inrange}) and combinators (\texttt{and}, \texttt{or}), offer a structured way of forming our queries over a set of clips (e.g. in a clip, did $2$ out balls \emph{and} $2$ wide balls occur?). We formalize this in Algorithm \ref{alg:query_form}.

\textbf{Step A: Creation of query set}

To construct a large set of diverse queries, we sample different lengths (\texttt{num\_joins}) for various queries. The length here refers to the number of operators being used for the formation of a particular query with the length parameter inducing complexity of 

To construct a large set of diverse queries, we apply our sets of operators and combinators on event chains, and pose them as a binary classification problem. For example, given an event chain $i$, our query may be \texttt{AND}(\texttt{atleast}(2 2's), \texttt{atleast}(1 wide)), which corresponds to a binary classification query asking if at least $2$ 2 runs and at least 1 wide ball occurred in the chain $i$. This procedure of generated queries easily generates thousands of queries using only simple event chains, and can easily extend beyond that using more complex combinations. 
% We first extract clips from cricket matches with lengths ranging from from 1 over ($\sim$5 minutes) to 10 overs ($\sim$50 minutes). To generate queries for these clips, we first note that a ball is an atomic unit in Cricket. Every ball corresponds to a certain event($n$ runs being scored, the batter getting out, the ball being bowled wide etc.). From these atomic events, we can form larger \textit{event chains}, which are an ordered set of atomic events; these event chains, combined with a set of logical operators, offer a structured way of forming our queries over a set of clips (e.g. in this clip, did $2$ out balls AND $2$ wide balls occur?).

\textbf{Creation of binary choice query set}

\textbf{Creation of multi-choice query set}
We also generate a set of multi-choice queries where the model is asked to output the number of occurrences of a chain of events (e.g. 4 THEN 0) within a timeframe and is given a set of options. To avoid over-counting, the ground-truth number is computed such that any two chains that are counted do not have overlapping timeframes. For example, if the query asks how many (4 THEN 0) occurred in an event chain of ‘4 4 0 0’, the correct answer is $1$. Queries were generally chosen such that no answer had more than a $50\%$ probability of occurring, and different queries were chosen for different query set buckets to ensure the model could not use the length of the given video clip as a learning signal.


\textbf{Step B: Evaluating Query Set on Event Chains}
Once a query is sampled of a particular length (\texttt{$num\_joins$}), we iterate over all the operators in the query to get ground truth evaluation for each operator. Hence, we instantiate operators using the set of atomic events ($A_{e}$) and also the numbers associated with them to act as thresholds for frequency of a particular operation occurence in the set. 


\textbf {Query set.} Within our dataset, we have a wide range of clip lengths to allow for varying levels of context localization and aggregation that models must learn to solve the dataset. To prevent models from using clip length to bias their outcomes, we form a \textit{query set} $Q = Q_1 \bigoplus Q_2 ... \bigoplus Q_n$ where $Q_1,...,Q_n$ are `buckets' of queries where only clips of a certain length are only paired with queries of a specific bucket. For our experiments, we use $n=5$ and divide the buckets such that queries from $Q_k$ are paired with clips that have between $2k-1$ and $2k$ overs in them. For example, queries from $Q_1$ are paired with clips that have 1-2 overs, while clips from $Q_5$ are paired with clips that have 9-10 overs.

% SHOW SEABORN DISTRIBUTION OF TIME IN CLIPS HERE%

\textbf{Training query set.} We observe that for our experiments, queries from the query formation process follow a long-tailed distribution in terms of occurrence, so we select a set of 30 binary-classification queries that occur with probability $0.5 \pm 0.05$ across \textit{all video clips} in their query set.

\input{sections/query_formation_algo}

% and generate a reference image. The pipeline uses this reference image to iterate over the video at a temporal granularity specified by the pipeline, using simple pixel-similarity metrics \todo{add the exact  equation here ig} and empirical thresholding \todo{here as well} to determine if each frame contains information about an "Over" and mapping the frame to its timestamp. Due to potential false detections in OCR and variable conditions in the video that may affect the scorecard, this whole process is nontrivial and requires extra steps for cleaning the annotations based on empirical observation of where these errors generally occur.



% \noindent \textbf{Step 1. Timestamp information using OCR:} Most cricket matches contain a spatially-fixed scorecard \todo{mark this in the fig} which contains information about which ball the match is at. The LCric pipeline first uses Google OCR Vision \todo{VM: Insert link} to locate the bounding box position of the "Overs" text in a few random frames of the video and generate a reference image. The pipeline uses this reference image to iterate over the video at a temporal granularity specified by the pipeline, using simple pixel-similarity metrics \todo{add the exact  equation here ig} and empirical thresholding \todo{here as well} to determine if each frame contains information about an "Over" and mapping the frame to its timestamp. Due to potential false detections in OCR and variable conditions in the video that may affect the scorecard, this whole process is nontrivial and requires extra steps for cleaning the annotations based on empirical observation of where these errors generally occur.
\\\\
% I think this part is unnecessary: It then crops out the bounding box and concatenates them into a large image before feeding several hundred frames of bounding boxes to a single OCR call to reduce the total number of OCR calls needed per video. Within this process, the timestamp of each crop is stored, so once all the OCR calls are finished, the first and last instance of a Ball/Over are used to determine the start and end timestamp of a specific Ball/Over. %
% \noindent \textbf{Stage 2. Mapping ESPNcricinfo to Timestamp Information:} Once we have our cricket match specified, we scrape commentary and other match event annotations from ESPNCricInfo. The ball-by-ball commentary generally contains information about which over and ball it is referring to, the batter, bowler, number of runs scored, and whether a ball was hit out or wide. In certain instances, the scraped information also contains actual text commentary about the match, which may be used in the future to generate different types of annotations for the matches. These annotations are aligned with the information from Stage 1, forming ball-by-ball annotations for each match.
\\\\
% \noindent \textbf{Stage 3. Creating Temporal-Varying Annotations:} The discrete nature of events within cricket allows combining several ball-level annotations into a single annotation spanning multiple balls to be actually meaningful. For example, asking if "batter $A$ scored a run on ball $10.1$" is a simple ball-level query that can be transformed into "did batter $A$ or $B$ score more over a series of contiguous balls" when ball-level annotations are concatenated. The LCric pipeline provides a script for generating annotations over any number of contiguous balls or overs at any specified density. 
\subsection{Dataset Statistics}
The dataset currently includes $1008$ hours of raw cricket matches across over $130$ unique matches. The current version includes $61957$ ball-by-ball annotations spanning 1 ball, 1 over, 2 overs, 5 overs, and 10 overs clips, where each over is roughly 5 minutes long, as shown in Figure \ref{fig:stats}. Figure \ref{fig:stats} also shows the number of clips in \lcric from 1 to 10 over videos, ranging from $10624$ 1-over clips to $1122$ 10-over clips. The videos are a fixed 360p resolution, although links to the source videos, which are of a higher resolution, will be provided as well. 
\\\\
We also observed that while the binary queries selected for the query train set are balanced when averaged across all matches, there is a considerable variance in their ground truth occurence probability across a match, as seen in Figure \ref{fig:stats}. We also note that most matches are viewed from the same camera angle, so it would be difficult for the model to attempt to use features within specific matches to exploit high variance queries. 
z
%% Caption: Figure X. Bottom: Clip length statistics for 1,6, and 10-over clips in LCric. Each over is on average 5 minutes. Top Left: Probability of any query in the train query set being true in each match over a 10-over period. Top Right: Number of annotations per time span


%%%%%%%%%%  make this another tex file firstly
% \section{Video Understanding Models on LCric}
% \subsection{Models}
% Video understanding models...
% % Talk about typical models %
% We experiment with \textbf{TQN}[cite] and \textbf{MeMViT}

% \textbf{Experiment setup.} Talk about dataset split here, how queries are fed, and the specifics of how the query set is done for train, val, test.

% Maybe add results here?


\subsection{\textbf{LCric's} Quality Check}
To verify that the annotations and clips in \lcric are accurate and clear respectively, we randomly sample $205$ clips from our dataset and ask human annotators on the AMT platform to label the events associated with each ball (number of runs, wide/out) and the timestamp at which it occurred. The latter is being asked to verify the over/ball timestamp bounds automatically generated by our method. 

\textcolor{red}{Timestamp annotations were marked correct if they occurred any where within the timestamp range of that ball.} Of the 1230 ball that were annotated, we report that $96.34\%$ of balls were correctly classified and $98.62\%$ of ball timestamps were correctly labelled. Additionally, $2.9\%$ of the clips were marked as either having incomplete information or being blurry. We found that this generally was due to confusion about the given instructions, which we further explain in the supplementary, along with other details regarding to the AMT setup (refer ex A.2).


%Additionally, $2.9\%$ of annotators had an incorrect labelling and indicated that there were some blurry parts or confusion regarding a missing ball, although this always occurred on a single ball and not the entire clip.


==> sections/query_formation_algo.tex <==
% \begin{wrapfigure}[20]{r}{0.52\textwidth}
% \vspace{-50pt}

% Ensure: O: operators {ATLEAST, ATMOST, INRANGE}
% Ensure: C: combinators {AND, OR}
% Require: E: list of all event chains
% Require: l: length of queries we want to generate
% Require: t: threshold probability

% # Generate all possible atomic queries
% initialize S to empty
% for all possible atomic events A_i do:
% 	for all integers n in [1,10] do:
% 		for all operators O_j do:
% 			Store triplet (O_j, n, A_u) in S

% Get all combinations P of Cartesian products (S_1 x S_2 x ... x S_l x C)

% # Compute occurrence of query in chains
% initialize Q to empty
% for all E_i do:
% 	for all P_j do:
% 		if AND in P_j and E_i satisfies all triplets in P_j:
% 			Q[P_j, E_i] = true
% 		else if OR in P_j and E_i satisfies any triplets in P_j:
% 			Q[P_j, E_i] = true
% 		else
% 			Q[P_j, E_i] = false

% # Prune any unwanted queries based on a threshold t
% initialize F to empty
% for all P_j:
% 	if percentage of occurrence P_j is  within [0.5-t,0.5+t], add to F

% return F

% \begin{algorithm}[H]
% \scriptsize
%   \caption{\small \label{alg:plan} Query Set Generation}
%     \begin{algorithmic}
%         \ENSURE $O$: operators $\{$ATLEAST, ATMOST, INRANGE$\}$ \\
%         \ENSURE $C$: combinators $\{$AND, OR$\}$ \\
%         \REQUIRE $E$: list of all event chains \\
%         \REQUIRE $l$: length of queries to generate \\
%         \REQUIRE $t$: confidence bound value for pruning queries \\
%     \end{algorithmic}
    
%     \textbf{initialize} $S$ to \textbf{empty} \Comment*[r]{Generate all possible atomic queries}
%     \For {all possible atomic events $A_i$ \textbf{do}:}{ 
%     	\For {all integers n in [1,10] \textbf{do}:} {
%     		\For {all operators $O_j$ \textbf{do}:} {
%     			Store triplet $(O_j, n, A_u)$ in $S$\; \Comment*[r]{This represents an atomic query, e.g. (ATLEAST, 1, wide)}
%     		}
%     	}
%     }
%     \textbf{Set} $P$ to be all combinations of Cartesian products $(S_1 \times S_2 \times ... \times S_l \times C)$ \Comment*[r]{Generate all combinations of atomic queries}
%     \textbf{initialize} $Q$ to \textbf{empty} \\
%     \For {all $E_i$ \textbf{do}:} {
%     	\For {all $P_j$ \textbf{do}:} {
%     	    \If {AND in $P_j$ and $E_i$ is \textbf{True} for all triplets in $P_j$:}{
%     	        $Q[P_j, E_i] = \text{\textbf{True}}$
%     	    }
%     		\If {OR in $P_j$ and $E_i$ is \textbf{True} for at least one triplet in $P_j$:}{
%     		    $Q[P_j, E_i] = \text{\textbf{True}}$
%     		}
%     		\Else{}{
%     			$Q[P_j, E_i] = \text{\textbf{False}}$
%     		}
%     	}
%     }
%     \textbf{initialize} $F$ to \textbf{empty} \Comment*[r]{Prune any unwanted queries based on a threshold $t$} \\
%     \For {all $P_j$ \textbf{do:}}{
%     	\If {$\%$ of occurrence $P_j$ is  within $[0.5-t,0.5+t]$} {add $P_j$ to $F$}
%     }
%     \Return{$F$}
% \end{algorithm}
%%

\begin{algorithm}[H]
\scriptsize
  \caption{\small \label{alg:plan} Query Set Generation}
  
  \label{alg:query_form}
%   \textcolor{black}{
%   \textbf{Set of operators:} \texttt{atleast()}, \texttt{atmost()}, \texttt{inrange()} \\
%   \textbf{Set of logical combinators:} \texttt{AND}, \texttt{OR} \\
%   \textbf{Set of event chains}: \texttt{$E_{c}$}
%   \\

%   \SetAlgoLined
  \var{\textcolor{gray}{\# The set of atomic events: [0,1,2,...,9,W,w]}} \\
  \textbf{Set of atomic events}: \texttt{$A_{e}$} 

  \var{\textcolor{gray}{\# The number of queries for the query set}} \\
  \textbf{Size of the query set}: \texttt{$n_q$} \\
  
%   \\ \\
%   \SetInd{0.2em}{0.5em}
    
    
    % \Function{qSetGen():}{ 
    
        % \For{i in \texttt{$E_{c}$ }}{
        
        \texttt{query\_set} = [] \\
        \For{\textnormal{\texttt{i}} in \textnormal{\texttt{range($n_q$)}}}{
            \\ 
            \var{\textbf{\textcolor{blue}{\# Step A: getting raw operators and combinators choice}}} \\
            \texttt{num\_joins} \sim [1,5]  \\
            \var{\textcolor{gray}{\# total length for operators set being sampled}} \\
            \var{\textcolor{gray}
            {for determining the query length}} 
            % \texttt{ops} \sim [\{\texttt{atleast()}, \texttt{atmost()}, \texttt{inrange()}\}, \texttt{num\_joints}]  ~~
            % \var{\textcolor{gray}{\# sampling operators list of the above sampled length}} \\
            % \texttt{combine\_op} \sim \{\texttt{AND}, \texttt{OR}\} ~~ \var{\textcolor{gray}{\# a sampled combinator for forming the query using the sampled operator set}} \\
            
            \texttt{ops} = \texttt{random.choices([\texttt{atleast()}, \texttt{atmost()}, \texttt{inrange()}], \texttt{num\_joins})} ~~ \var{\textcolor{gray}{\# sampling list of operators}} \\
            \texttt{combine\_op} = \texttt{random.choices([\texttt{and}, \texttt{or}], 1)} ~~ \var{\textcolor{gray}{\# sampling the combination operator}} \\
            
            
            \var{\textbf{\textcolor{blue}{\# Step B: instantiating a query for query set for \patmatch }}}\\
            \var{\texttt{query} = []}\\
            \For{\textnormal{\texttt{op}} in \textnormal{\texttt{ops}} }{
                
                \\
                \var{\textcolor{gray}{\# specify lower bound for atleast/inrange ops}} \\
                \texttt{occ\_min} \sim [1,10]  ~~ \\
                \var{\textcolor{gray}{\# specify upper bound bound for atmost/inrange ops}} \\
                \texttt{occ\_max} \sim [\texttt{occ\_min},10] ~~ \\
                \var{\textcolor{gray}{\# sample atomic events in query}} \\
                \texttt{atomic\_event} \sim [\texttt{$A_{e}$}] ~~  \\
                
                \var{\textcolor{gray}{\# Using the above variables for defining an occurence pattern for atomic\_event}}
                
                \texttt{instanced\_op} = \texttt{op}(\texttt{occ\_min}, \texttt{occ\_max}, \texttt{atomic\_event})
                
                
                % \If{j \textbf{is} \texttt{atleast} }{
                    
                %     \texttt{instanced\_op} = \texttt{atleast(\texttt{occ\_min}, \texttt{atomic\_event})}  ~~ \var{\textcolor{gray}{\# instantiating the \texttt{atleast} operator}} \\
                %     \var{\textcolor{cyan}{\# Eg format for instanced\_op `\texttt{atleast} [\texttt{occ\_min}] [\texttt{atomic\_event}]'}} \\
                    
                % }
                
                % \If{j \textbf{is} \texttt{atmost} }{
                    
                %     \texttt{instanced\_op} = \texttt{atmost(\texttt{occ\_max}, \texttt{atomic\_event})}  ~~ \var{\textcolor{gray}{\# instantiating the \texttt{atmost} operator}} \\
                %     \var{\textcolor{cyan}{\# Eg format for instanced\_op `\texttt{atmost} [\texttt{occ\_max}] [\texttt{atomic\_event}]'}} \\
                
                % }
                
                % \If{j \textbf{is} \texttt{inrange} }{
                    
                %     \texttt{instanced\_op} = \texttt{inrange(\texttt{occ\_min}, \texttt{occ\_max}, \texttt{atomic\_event})}  ~~ \var{\textcolor{gray}{\# instantiating the \texttt{inrange} operator}} \\
                %     \var{\textcolor{cyan}{\# Eg format for instanced\_op `\texttt{inrange} [\texttt{occ\_min}, \texttt{occ\_max}] [\texttt{atomic\_event}]'}} \\
                
                % }
                
                % \texttt{eval} = \texttt{instanced\_op}(i) ~~ \var{\textcolor{gray}{\# evaluating on the current event chain using the instantiated operator}} \\
                \texttt{query.append(\texttt{instanced\_op})} \\
                
                
            }
            
            \texttt{final\_query} = \texttt{join\_op(query)}
            
            \texttt{query\_set.append(\texttt{final\_query})} \\
            
            }
                
            % \texttt{final\_eval} = [\texttt{eval\_gt}, \texttt{join\_op}] ~~ \var{\textcolor{gray}{\# combining the different operators result using the sampled combinator}} \\
            
            
        % }
    
        
    % }
    
\end{algorithm}


% \var{\textcolor{gray}{\# nothing to rearrange}} \\
            % \If{not \texttt{R}.rearrangements():}{
            %     \var{\textcolor{gray}{\# explore for n$_e$ steps}} \\
            %     \For{i in range(n$_e$):}{
            %         \var{\textcolor{gray}{\# take an exploration step}} \\
            %         \var{obs = \ttE.act(M, N)} \\
            %         \var{\textcolor{gray}{\# update map and rearrange modules}} \\
            %         \var{M.update(obs); R.update(obs)} \\
            %     }
            %     \var{t = t + n$_e$} \\
            %     \var{R.rescore(L)}~~\var{\textcolor{gray}{\# update scores using L}}
            % }
            % \Else{:}{
            %     \var{\textcolor{gray}{\# rearrange until finished}} \\
            %     \For{r in R.rearrangements():}{
            %         \var{\textcolor{gray}{\# object and correct receptacle}} \\
            %         \var{obj,rec = r.obj,r.rec} \\
            %         \var{\textcolor{gray}{\# nav \& pick obj, then nav \& place on rec}} \\
            %         \If{N.nav(obj) \& P.pick(obj) \& N.nav(rec) \& P.place(obj, rec):}{\var{M.update(obs); R.update(obs)}}
            %         \var{t = t+n$_r$} \var{\textcolor{gray}{\# update steps}} \\
            %     }
            % }

% \end{wrapfigure}

==> tables/atomic_events.tex <==
\begin{table}[t]
\vspace{-9pt}
    \caption{\small{The 12 atomic events that we use to build the query set for our dataset.}}
    \vspace{-10pt}
    \scriptsize
    \begin{center}
		\setlength{\tabcolsep}{2pt}
		\begin{tabular}{| p{1.5cm} | p{4.5cm} |}
			\toprule
            \textbf{Atomic Events} & \textbf{Description}
            \\
            \midrule
            0,1,2, ...,8,9 & Possible number of runs scored in a single ball
            \\
            \midrule
            W & Wicket being taken (the current batsman gets out)
            \\
            \midrule
            w & Wide ball (a foul leading to an extra run and ball given to batting team)
            \\
            \bottomrule
		\end{tabular}
	\end{center}
	\label{tab:atomic_events}
\end{table}

==> tables/human_annotation.tex <==
\begin{table*}[t!]
    % \vspace{-20pt}
	\setlength{\tabcolsep}{3pt}
	\caption{
    \small
    Human annotator performance on 1-over query set vs. baseline models.
    \var{QS Acc}: Accuracy on 1-over query set.
    }
    \begin{center}
    \resizebox{0.5\linewidth}{!}{
    		\begin{tabular}{c c l l cc cc cc cc}
    		    \toprule
    		    & 
    			\multicolumn{1}{c}{\scriptsize\textbf{Human Annotators}} & & \multicolumn{1}{c}{\scriptsize\textbf{TQN}} & & \multicolumn{1}{c}{\scriptsize\textbf{MeMViT}} & \\
    			\cmidrule(r){1-7}
            \scriptsize\texttt{\textbf{QS Acc}} & \footnotesize 96.53 & & \footnotesize 70.16 & & \footnotesize 67.98 \\
            \hline
    		\end{tabular}
    	}
    \end{center}
	
	\label{table:humans}
\vspace{-10pt}
\end{table*}


% % HUMAN BASELINE NUMBERS. Query set accuracy: 96.53 %
% % Per-ball annotation accuracy: 96.34 and Per-ball timestamp accuracy: 98.62  %

==> utils/custom_packages.tex <==
% \usepackage{epsfig}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{subcaption}

% \usepackage{hyperref}
\usepackage{cleveref}
\usepackage{caption}
\usepackage{textcomp}
\usepackage{stmaryrd}
\usepackage{upgreek}
\usepackage{bm}
\usepackage{cases}
\usepackage{mathtools}
\usepackage{multirow}
\usepackage{bbm}
\usepackage{romannum}

\usepackage{paralist}
\usepackage{enumitem}

\usepackage{cite}

\usepackage{multirow}
\usepackage{rotating}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{tabulary}
\usepackage{xcolor,colortbl}

\usepackage{pifont}


==> utils/macros.tex <==
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\st{s.t\onedot} \def\St{\emph{S.t}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
% \makeatother

% Color Annotation
\definecolor{curve-blue}{rgb}{0.0, 0.2, 0.7}
\definecolor{curve-orange}{rgb}{0.9,0.2,0.0}
\definecolor{curve-green}{rgb}{0.1,0.5,0.0}
\newcommand{\var}{\texttt}

\newcommand{\lcric}{{LCric}\xspace}
\newcommand{\lcricm}{{LCric-Mini}\xspace}
\newcommand{\cric}{Cricket\xspace}
\newcommand{\LVU}{LVU\xspace}
\newcommand{\ASAP}{ASAP\xspace}
\newcommand{\patmatch}{\texttt{??}}
\newcommand{\metadata}{\textit{match state}\xspace}

\newcommand{\todo}[1]{{\color{red} [TODO: #1]}} 
\newcommand{\kn}[1]{{\color{magenta} [KN: #1]}} 
\newcommand{\yk}[1]{{\color{teal}#1 --- YK}} 
\newcommand{\vm}[1]{{\color{blue} [VM: #1]}}
\newcommand{\ani}[1]{{\color{cyan} [AA: #1]}}





%%%% Yash: The macros below can be useful, but not all of them are needed so commented out. 

% \parskip=5pt
% \abovedisplayskip 3.0pt plus2pt minus2pt%
% \belowdisplayskip \abovedisplayskip
% \renewcommand{\baselinestretch}{1} %

% \newcommand{\csection}[1]{
%     \vspace{-0.13in}
%     \section{#1}
%     \vspace{-0.13in}
% }

% \newcommand{\csubsection}[1]{
%     \vspace{-0.12in}
%     \subsection{#1}
%     \vspace{-0.10in}
% }

% \newcommand{\csubsubsection}[1]{
%     \vspace{-0.06in}
%     \subsubsection{#1}
%     \vspace{-0.05in}
% }


% \setlength{\floatsep}{1ex plus 0ex minus 0.5ex}
% \setlength{\textfloatsep}{3ex plus 0ex minus 0ex}
% \setlength{\abovecaptionskip}{0ex plus 0ex minus 0ex}
% \setlength{\belowcaptionskip}{0ex plus 0ex minus 0ex}


% \newcommand{\cmark}{\ding{51}}%
% \newcommand{\xmark}{\ding{55}}%
% \newcommand{\band}{\rowcolor{gray!10}}


% \newenvironment{compitemize} {
% \begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=*] \renewcommand\labelitemi{$\bullet$}
% }   {\end{itemize}}


% \newenvironment{compenumerate} {\begin{enumerate}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=*]}   {\end{enumerate}}

% \newcommand{\confint}[1]{\scriptsize $\pm$ #1 }

% \usepackage{inconsolata}
% \newcommand{\ttbf}[1]{\texttt{\textbf{#1}}}
% \newcommand{\fwd}[0]{\texttt{MOVE\_FORWARD}\xspace}
% \newcommand{\turnr}[0]{\texttt{TURN\_RIGHTt}\xspace}
% \newcommand{\turnl}[0]{\texttt{TURN\_LEFT}\xspace}
% \newcommand{\grab}[0]{\texttt{GRAB\_RELEASE}\xspace}
% \newcommand{\plasma}[0]{\textbf{\texttt{PLASMA}}\xspace}

% \newcommand{\algoref}[1]{Algo\onedot~\ref{#1}}
% \newcommand{\thmref}[1]{Theorem~\ref{#1}}
% \newcommand{\prgref}[1]{Program~\ref{#1}}
% \newcommand{\clmref}[1]{Claim~\ref{#1}}
% \newcommand{\lemref}[1]{Lemma~\ref{#1}}
% \newcommand{\ptyref}[1]{Property~\ref{#1}}
% \newcommand{\defref}[1]{Definition~\ref{#1}}
% \newcommand{\appref}[1]{Appendix~\ref{#1}}
% \newcommand{\lstref}[1]{Listing~\ref{#1}}

% \newcommand{\tname}{Housekeep\xspace}
% \newcommand{\rlmethod}{end-to-end\xspace}
% \newcommand{\ajs}[1]{{\color{red}{(\textbf{Andrew: }#1)}}}
% \newcommand{\sy}[1]{{\color{blue}{(\textbf{Sriram: }#1)}}}
% \newcommand{\arun}[1]{{\color{purple}{(\textbf{Arun: }#1)}}}

% \newcommand{\interactdist}{$0.25m$\xspace}
% \newcommand{\numreceptacles}{$X$\xspace}
% \newcommand{\numrooms}{$105$\xspace}

% \newcommand{\recmodels}{$395$\xspace}
% \newcommand{\reccats}{$32$\xspace}
% \newcommand{\roomrecs}{$128$\xspace}

% \newcommand{\objmodels}{$1801$\xspace}
% \newcommand{\objcats}{$269$\xspace}




% \newcommand\todo[1]{\textcolor{red}{#1}}
% \newcommand\ha[1]{\textcolor{orange}{HA: #1}}
% \newcommand\as[1]{\textcolor{magenta}{AS: #1}}
% \newcommand\yk[1]{\textcolor{green}{#1}}
% \newcommand\sry[1]{\textcolor{brown}{HA: #1}}
% \newcommand\ar[1]{\textcolor{pink}{AR: #1}}







% \usepackage{amsmath,amsfonts,bm}

% \newcommand{\figleft}{{\em (Left)}}
% \newcommand{\figcenter}{{\em (Center)}}
% \newcommand{\figright}{{\em (Right)}}
% \newcommand{\figtop}{{\em (Top)}}
% \newcommand{\figbottom}{{\em (Bottom)}}
% \newcommand{\captiona}{{\em (a)}}
% \newcommand{\captionb}{{\em (b)}}
% \newcommand{\captionc}{{\em (c)}}
% \newcommand{\captiond}{{\em (d)}}

% \newcommand{\newterm}[1]{{\bf #1}}


% \def\figref#1{figure~\ref{#1}}
% \def\Figref#1{Fig\onedot~\ref{#1}}
% \def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
% \def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% \def\secref#1{section~\ref{#1}}
% \def\Secref#1{Section~\ref{#1}}
% \def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% \def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% \def\eqref#1{equation~\ref{#1}}
% \def\Eqref#1{Equation~\ref{#1}}
% \def\plaineqref#1{\ref{#1}}
% \def\chapref#1{chapter~\ref{#1}}
% \def\Chapref#1{Chapter~\ref{#1}}
% \def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% \def\algref#1{algorithm~\ref{#1}}
% \def\Algref#1{Algorithm~\ref{#1}}
% \def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
% \def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% \def\partref#1{part~\ref{#1}}
% \def\Partref#1{Part~\ref{#1}}
% \def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

% \def\myquote#1{\emph{`#1'}}
% \def\ceil#1{\lceil #1 \rceil}
% \def\floor#1{\lfloor #1 \rfloor}
% \def\1{\bm{1}}
% \newcommand{\train}{\mathcal{D}}
% \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

% \def\eps{{\epsilon}}


% \def\reta{{\textnormal{$\eta$}}}
% \def\ra{{\textnormal{a}}}
% \def\rb{{\textnormal{b}}}
% \def\rc{{\textnormal{c}}}
% \def\rd{{\textnormal{d}}}
% \def\re{{\textnormal{e}}}
% \def\rf{{\textnormal{f}}}
% \def\rg{{\textnormal{g}}}
% \def\rh{{\textnormal{h}}}
% \def\ri{{\textnormal{i}}}
% \def\rj{{\textnormal{j}}}
% \def\rk{{\textnormal{k}}}
% \def\rl{{\textnormal{l}}}
% \def\rn{{\textnormal{n}}}
% \def\ro{{\textnormal{o}}}
% \def\rp{{\textnormal{p}}}
% \def\rq{{\textnormal{q}}}
% \def\rr{{\textnormal{r}}}
% \def\rs{{\textnormal{s}}}
% \def\rt{{\textnormal{t}}}
% \def\ru{{\textnormal{u}}}
% \def\rv{{\textnormal{v}}}
% \def\rw{{\textnormal{w}}}
% \def\rx{{\textnormal{x}}}
% \def\ry{{\textnormal{y}}}
% \def\rz{{\textnormal{z}}}

% \def\rvepsilon{{\mathbf{\epsilon}}}
% \def\rvtheta{{\mathbf{\theta}}}
% \def\rva{{\mathbf{a}}}
% \def\rvb{{\mathbf{b}}}
% \def\rvc{{\mathbf{c}}}
% \def\rvd{{\mathbf{d}}}
% \def\rve{{\mathbf{e}}}
% \def\rvf{{\mathbf{f}}}
% \def\rvg{{\mathbf{g}}}
% \def\rvh{{\mathbf{h}}}
% \def\rvu{{\mathbf{i}}}
% \def\rvj{{\mathbf{j}}}
% \def\rvk{{\mathbf{k}}}
% \def\rvl{{\mathbf{l}}}
% \def\rvm{{\mathbf{m}}}
% \def\rvn{{\mathbf{n}}}
% \def\rvo{{\mathbf{o}}}
% \def\rvp{{\mathbf{p}}}
% \def\rvq{{\mathbf{q}}}
% \def\rvr{{\mathbf{r}}}
% \def\rvs{{\mathbf{s}}}
% \def\rvt{{\mathbf{t}}}
% \def\rvu{{\mathbf{u}}}
% \def\rvv{{\mathbf{v}}}
% \def\rvw{{\mathbf{w}}}
% \def\rvx{{\mathbf{x}}}
% \def\rvy{{\mathbf{y}}}
% \def\rvz{{\mathbf{z}}}

% \def\erva{{\textnormal{a}}}
% \def\ervb{{\textnormal{b}}}
% \def\ervc{{\textnormal{c}}}
% \def\ervd{{\textnormal{d}}}
% \def\erve{{\textnormal{e}}}
% \def\ervf{{\textnormal{f}}}
% \def\ervg{{\textnormal{g}}}
% \def\ervh{{\textnormal{h}}}
% \def\ervi{{\textnormal{i}}}
% \def\ervj{{\textnormal{j}}}
% \def\ervk{{\textnormal{k}}}
% \def\ervl{{\textnormal{l}}}
% \def\ervm{{\textnormal{m}}}
% \def\ervn{{\textnormal{n}}}
% \def\ervo{{\textnormal{o}}}
% \def\ervp{{\textnormal{p}}}
% \def\ervq{{\textnormal{q}}}
% \def\ervr{{\textnormal{r}}}
% \def\ervs{{\textnormal{s}}}
% \def\ervt{{\textnormal{t}}}
% \def\ervu{{\textnormal{u}}}
% \def\ervv{{\textnormal{v}}}
% \def\ervw{{\textnormal{w}}}
% \def\ervx{{\textnormal{x}}}
% \def\ervy{{\textnormal{y}}}
% \def\ervz{{\textnormal{z}}}

% \def\rmA{{\mathbf{A}}}
% \def\rmB{{\mathbf{B}}}
% \def\rmC{{\mathbf{C}}}
% \def\rmD{{\mathbf{D}}}
% \def\rmE{{\mathbf{E}}}
% \def\rmF{{\mathbf{F}}}
% \def\rmG{{\mathbf{G}}}
% \def\rmH{{\mathbf{H}}}
% \def\rmI{{\mathbf{I}}}
% \def\rmJ{{\mathbf{J}}}
% \def\rmK{{\mathbf{K}}}
% \def\rmL{{\mathbf{L}}}
% \def\rmM{{\mathbf{M}}}
% \def\rmN{{\mathbf{N}}}
% \def\rmO{{\mathbf{O}}}
% \def\rmP{{\mathbf{P}}}
% \def\rmQ{{\mathbf{Q}}}
% \def\rmR{{\mathbf{R}}}
% \def\rmS{{\mathbf{S}}}
% \def\rmT{{\mathbf{T}}}
% \def\rmU{{\mathbf{U}}}
% \def\rmV{{\mathbf{V}}}
% \def\rmW{{\mathbf{W}}}
% \def\rmX{{\mathbf{X}}}
% \def\rmY{{\mathbf{Y}}}
% \def\rmZ{{\mathbf{Z}}}

% \def\ermA{{\textnormal{A}}}
% \def\ermB{{\textnormal{B}}}
% \def\ermC{{\textnormal{C}}}
% \def\ermD{{\textnormal{D}}}
% \def\ermE{{\textnormal{E}}}
% \def\ermF{{\textnormal{F}}}
% \def\ermG{{\textnormal{G}}}
% \def\ermH{{\textnormal{H}}}
% \def\ermI{{\textnormal{I}}}
% \def\ermJ{{\textnormal{J}}}
% \def\ermK{{\textnormal{K}}}
% \def\ermL{{\textnormal{L}}}
% \def\ermM{{\textnormal{M}}}
% \def\ermN{{\textnormal{N}}}
% \def\ermO{{\textnormal{O}}}
% \def\ermP{{\textnormal{P}}}
% \def\ermQ{{\textnormal{Q}}}
% \def\ermR{{\textnormal{R}}}
% \def\ermS{{\textnormal{S}}}
% \def\ermT{{\textnormal{T}}}
% \def\ermU{{\textnormal{U}}}
% \def\ermV{{\textnormal{V}}}
% \def\ermW{{\textnormal{W}}}
% \def\ermX{{\textnormal{X}}}
% \def\ermY{{\textnormal{Y}}}
% \def\ermZ{{\textnormal{Z}}}


% \def\evalpha{{\alpha}}
% \def\evbeta{{\beta}}
% \def\evepsilon{{\epsilon}}
% \def\evlambda{{\lambda}}
% \def\evomega{{\omega}}
% \def\evmu{{\mu}}
% \def\evpsi{{\psi}}
% \def\evsigma{{\sigma}}
% \def\evtheta{{\theta}}
% \def\eva{{a}}
% \def\evb{{b}}
% \def\evc{{c}}
% \def\evd{{d}}
% \def\eve{{e}}
% \def\evf{{f}}
% \def\evg{{g}}
% \def\evh{{h}}
% \def\evi{{i}}
% \def\evj{{j}}
% \def\evk{{k}}
% \def\evl{{l}}
% \def\evm{{m}}
% \def\evn{{n}}
% \def\evo{{o}}
% \def\evp{{p}}
% \def\evq{{q}}
% \def\evr{{r}}
% \def\evs{{s}}
% \def\evt{{t}}
% \def\evu{{u}}
% \def\evv{{v}}
% \def\evw{{w}}
% \def\evx{{x}}
% \def\evy{{y}}
% \def\evz{{z}}

% \def\mA{{\bm{A}}}
% \def\mB{{\bm{B}}}
% \def\mC{{\bm{C}}}
% \def\mD{{\bm{D}}}
% \def\mE{{\bm{E}}}
% \def\mF{{\bm{F}}}
% \def\mG{{\bm{G}}}
% \def\mH{{\bm{H}}}
% \def\mI{{\bm{I}}}
% \def\mJ{{\bm{J}}}
% \def\mK{{\bm{K}}}
% \def\mL{{\bm{L}}}
% \def\mM{{\bm{M}}}
% \def\mN{{\bm{N}}}
% \def\mO{{\bm{O}}}
% \def\mP{{\bm{P}}}
% \def\mQ{{\bm{Q}}}
% \def\mR{{\bm{R}}}
% \def\mS{{\bm{S}}}
% \def\mT{{\bm{T}}}
% \def\mU{{\bm{U}}}
% \def\mV{{\bm{V}}}
% \def\mW{{\bm{W}}}
% \def\mX{{\bm{X}}}
% \def\mY{{\bm{Y}}}
% \def\mZ{{\bm{Z}}}
% \def\mBeta{{\bm{\beta}}}
% \def\mPhi{{\bm{\Phi}}}
% \def\mLambda{{\bm{\Lambda}}}
% \def\mSigma{{\bm{\Sigma}}}

% \DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
% \SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
% \newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
% \def\tA{{\tens{A}}}
% \def\tB{{\tens{B}}}
% \def\tC{{\tens{C}}}
% \def\tD{{\tens{D}}}
% \def\tE{{\tens{E}}}
% \def\tF{{\tens{F}}}
% \def\tG{{\tens{G}}}
% \def\tH{{\tens{H}}}
% \def\tI{{\tens{I}}}
% \def\tJ{{\tens{J}}}
% \def\tK{{\tens{K}}}
% \def\tL{{\tens{L}}}
% \def\tM{{\tens{M}}}
% \def\tN{{\tens{N}}}
% \def\tO{{\tens{O}}}
% \def\tP{{\tens{P}}}
% \def\tQ{{\tens{Q}}}
% \def\tR{{\tens{R}}}
% \def\tS{{\tens{S}}}
% \def\tT{{\tens{T}}}
% \def\tU{{\tens{U}}}
% \def\tV{{\tens{V}}}
% \def\tW{{\tens{W}}}
% \def\tX{{\tens{X}}}
% \def\tY{{\tens{Y}}}
% \def\tZ{{\tens{Z}}}


% \def\gA{{\mathcal{A}}}
% \def\gB{{\mathcal{B}}}
% \def\gC{{\mathcal{C}}}
% \def\gD{{\mathcal{D}}}
% \def\gE{{\mathcal{E}}}
% \def\gF{{\mathcal{F}}}
% \def\gG{{\mathcal{G}}}
% \def\gH{{\mathcal{H}}}
% \def\gI{{\mathcal{I}}}
% \def\gJ{{\mathcal{J}}}
% \def\gK{{\mathcal{K}}}
% \def\gL{{\mathcal{L}}}
% \def\gM{{\mathcal{M}}}
% \def\gN{{\mathcal{N}}}
% \def\gO{{\mathcal{O}}}
% \def\gP{{\mathcal{P}}}
% \def\gQ{{\mathcal{Q}}}
% \def\gR{{\mathcal{R}}}
% \def\gS{{\mathcal{S}}}
% \def\gT{{\mathcal{T}}}
% \def\gU{{\mathcal{U}}}
% \def\gV{{\mathcal{V}}}
% \def\gW{{\mathcal{W}}}
% \def\gX{{\mathcal{X}}}
% \def\gY{{\mathcal{Y}}}
% \def\gZ{{\mathcal{Z}}}

% \def\sA{{\mathbb{A}}}
% \def\sB{{\mathbb{B}}}
% \def\sC{{\mathbb{C}}}
% \def\sD{{\mathbb{D}}}
% \def\sF{{\mathbb{F}}}
% \def\sG{{\mathbb{G}}}
% \def\sH{{\mathbb{H}}}
% \def\sI{{\mathbb{I}}}
% \def\sJ{{\mathbb{J}}}
% \def\sK{{\mathbb{K}}}
% \def\sL{{\mathbb{L}}}
% \def\sM{{\mathbb{M}}}
% \def\sN{{\mathbb{N}}}
% \def\sO{{\mathbb{O}}}
% \def\sP{{\mathbb{P}}}
% \def\sQ{{\mathbb{Q}}}
% \def\sR{{\mathbb{R}}}
% \def\sS{{\mathbb{S}}}
% \def\sT{{\mathbb{T}}}
% \def\sU{{\mathbb{U}}}
% \def\sV{{\mathbb{V}}}
% \def\sW{{\mathbb{W}}}
% \def\sX{{\mathbb{X}}}
% \def\sY{{\mathbb{Y}}}
% \def\sZ{{\mathbb{Z}}}

% \def\emLambda{{\Lambda}}
% \def\emA{{A}}
% \def\emB{{B}}
% \def\emC{{C}}
% \def\emD{{D}}
% \def\emE{{E}}
% \def\emF{{F}}
% \def\emG{{G}}
% \def\emH{{H}}
% \def\emI{{I}}
% \def\emJ{{J}}
% \def\emK{{K}}
% \def\emL{{L}}
% \def\emM{{M}}
% \def\emN{{N}}
% \def\emO{{O}}
% \def\emP{{P}}
% \def\emQ{{Q}}
% \def\emR{{R}}
% \def\emS{{S}}
% \def\emT{{T}}
% \def\emU{{U}}
% \def\emV{{V}}
% \def\emW{{W}}
% \def\emX{{X}}
% \def\emY{{Y}}
% \def\emZ{{Z}}
% \def\emSigma{{\Sigma}}

% \newcommand{\etens}[1]{\mathsfit{#1}}
% \def\etLambda{{\etens{\Lambda}}}
% \def\etA{{\etens{A}}}
% \def\etB{{\etens{B}}}
% \def\etC{{\etens{C}}}
% \def\etD{{\etens{D}}}
% \def\etE{{\etens{E}}}
% \def\etF{{\etens{F}}}
% \def\etG{{\etens{G}}}
% \def\etH{{\etens{H}}}
% \def\etI{{\etens{I}}}
% \def\etJ{{\etens{J}}}
% \def\etK{{\etens{K}}}
% \def\etL{{\etens{L}}}
% \def\etM{{\etens{M}}}
% \def\etN{{\etens{N}}}
% \def\etO{{\etens{O}}}
% \def\etP{{\etens{P}}}
% \def\etQ{{\etens{Q}}}
% \def\etR{{\etens{R}}}
% \def\etS{{\etens{S}}}
% \def\etT{{\etens{T}}}
% \def\etU{{\etens{U}}}
% \def\etV{{\etens{V}}}
% \def\etW{{\etens{W}}}
% \def\etX{{\etens{X}}}
% \def\etY{{\etens{Y}}}
% \def\etZ{{\etens{Z}}}

% \newcommand{\pdata}{p_{\rm{data}}}
% \newcommand{\ptrain}{\hat{p}_{\rm{data}}}
% \newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% \newcommand{\pmodel}{p_{\rm{model}}}
% \newcommand{\Pmodel}{P_{\rm{model}}}
% \newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% \newcommand{\pencode}{p_{\rm{encoder}}}
% \newcommand{\pdecode}{p_{\rm{decoder}}}
% \newcommand{\precons}{p_{\rm{reconstruct}}}

% \newcommand{\laplace}{\mathrm{Laplace}} %

% \newcommand{\E}{\mathbb{E}}
% \newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\emp}{\tilde{p}}
% \newcommand{\lr}{\alpha}
% \newcommand{\reg}{\lambda}
% \newcommand{\rect}{\mathrm{rectifier}}
% \newcommand{\softmax}{\mathrm{softmax}}
% \newcommand{\sigmoid}{\sigma}
% \newcommand{\softplus}{\zeta}
% \newcommand{\KL}{D_{\mathrm{KL}}}
% \newcommand{\Var}{\mathrm{Var}}
% \newcommand{\standarderror}{\mathrm{SE}}
% \newcommand{\Cov}{\mathrm{Cov}}
% \newcommand{\normlzero}{L^0}
% \newcommand{\normlone}{L^1}
% \newcommand{\normltwo}{L^2}
% \newcommand{\normlp}{L^p}
% \newcommand{\normmax}{L^\infty}

% \newcommand{\parents}{Pa} %

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
% \let\ab\allowbreak





% \newcommand{\embeds}[1]{\;\lhook\joinrel\xrightarrow{#1}\;}

% \newcommand{\ds}{\displaystyle}
% \newcommand{\bs}{\boldsymbol}
% \renewcommand{\th}{\ensuremath{^{\mathrm{th}}}~}




% \def\naive{na\"\i ve\xspace}
% \def\naively{na\"\i vely\xspace}
% \def\Naive{Na\"\i ve\xspace}
% \def\Naively{Na\"\i vely\xspace}


% \makeatletter
% \newcommand{\bfgreek}[1]{\bm{\@nameuse{#1}}}
% \makeatother

% \newcommand{\ind}[1]{[\hspace{-1pt}[#1]\hspace{-1pt}] }
% \newcommand{\red}[1]{\textcolor{red}{#1}}

% \newcommand{\norm}[1]{\left| \hspace{-0.7pt}\left|#1\right| \hspace{-0.7pt}\right|}


% \newcommand{\beginsupplement}{
%     \setcounter{table}{0}
%     \renewcommand{\thetable}{S\arabic{table}}%
%     \setcounter{figure}{0}
%     \renewcommand{\thefigure}{S\arabic{figure}}%
%     \setcounter{equation}{0}
%     \renewcommand{\theequation}{S\arabic{equation}}
% }


% \newcommand{\al}{\alpha}
% \newcommand{\be}{\beta}
% \newcommand{\Gm}{\Gamma}
% \newcommand{\gm}{\gamma}
% \newcommand{\De}{\Delta}
% \newcommand{\de}{\delta}
% \newcommand{\ve}{\varepsilon}
% \newcommand{\ka}{\kappa}
% \newcommand{\La}{\Lambda}
% \newcommand{\la}{\lambda}
% \providecommand{\Si}{\Sigma} %
% \providecommand{\si}{\sigma}
% \newcommand{\ta}{\tau}
% \newcommand{\Te}{\Theta}
% \newcommand{\te}{\theta}
% \newcommand{\Ph}{\Phi}
% \newcommand{\ph}{\varphi}
% \newcommand{\Ps}{\Psi}
% \newcommand{\ps}{\psi}
% \newcommand{\om}{\omega}
% \newcommand{\Om}{\Omega}


% \newcommand{\mcA}{\mathcal{A}}
% \newcommand{\mcB}{\mathcal{B}}
% \newcommand{\mcC}{\mathcal{C}}
% \newcommand{\mcD}{\mathcal{D}}
% \newcommand{\mcE}{\mathcal{E}}
% \newcommand{\mcF}{\mathcal{F}}
% \newcommand{\mcG}{\mathcal{G}}
% \newcommand{\mcJ}{\mathcal{J}}
% \newcommand{\mcL}{\mathcal{L}}
% \newcommand{\mcO}{\mathcal{O}}
% \newcommand{\mcP}{\mathcal{P}}
% \newcommand{\mcT}{\mathcal{T}}
% \newcommand{\mcU}{\mathcal{U}}
% \newcommand{\mcW}{\mathcal{W}}
% \newcommand{\mcR}{\mathcal{R}}

% \newcommand{\rmi}{\mathrm{i}}
% \newcommand{\rmj}{\mathrm{j}}
% \newcommand{\rmk}{\mathrm{k}}


% \newcommand{\ttL}{\texttt{L}}
% \newcommand{\ttE}{\texttt{E}}
% \newcommand{\ttM}{\texttt{M}}
% \newcommand{\ttR}{\texttt{R}}
% \newcommand{\ttP}{\texttt{P}}
% \newcommand{\ttN}{\texttt{N}}



% \renewcommand{\KwSty}[1]{\textnormal{\textcolor{blue!90!black}{\ttfamily #1}}\unskip}
% \renewcommand{\ArgSty}[1]{\textnormal{\ttfamily #1}\unskip}
% \SetKwComment{Comment}{\color{green!50!black}// }{}
% \renewcommand{\CommentSty}[1]{\textnormal{\ttfamily\color{green!50!black}#1}\unskip}
% \newcommand{\assign}{\leftarrow}
% \newcommand{\FuncCall}[2]{\texttt{ #1(#2)}}
% \SetKwProg{Function}{def}{}{}
% \renewcommand{\ProgSty}[1]{\texttt{ #1}}
% \SetKwProg{Class}{class}{}{}

% \SetKwProg{While}{while}{}{}
% \SetKwProg{For}{for}{}{}
% \SetKwProg{If}{if}{}{}
% \SetKwProg{Else}{else}{\unskip}{}


% \newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}

% \usepackage{booktabs}       %
% \usepackage{amsfonts}       %
% \usepackage{nicefrac}       %
% \usepackage{microtype}      %
% \usepackage{colortbl}
% \usepackage{placeins}

% \usepackage{float}
% \usepackage{fontawesome}
% \usepackage{adjustbox}
% \newcolumntype{R}[2]{%
%     >{\adjustbox{angle=#1,lap=\width-(#2)}\bgroup}%
%     l%
%     <{\egroup}%
% }
% \newcommand*\rot{\multicolumn{1}{R{30}{1em}}}
% \usepackage{rotating}
% \newcommand{\lcric}{\emph{LCric}}
% \newcommand{\lcricm}{\emph{LCric-500}}


